A sub-quadratic algorithm for the longest common increasing subsequence problem

The Longest Common Increasing Subsequence problem (LCIS) is a natural variant of the celebrated Longest Common Subsequence (LCS) problem. For LCIS, as well as for LCS, there is an $O(n^2)$-time algorithm and a SETH-based conditional lower bound of $O(n^{2-\varepsilon})$. For LCS, there is also the Masek-Paterson $O(n^2 / \log{n})$-time algorithm, which does not seem to adapt to LCIS in any obvious way. Hence, a natural question arises: does any (slightly) sub-quadratic algorithm exist for the Longest Common Increasing Subsequence problem? We answer this question positively, presenting a $O(n^2 / \log^a{n})$-time algorithm for $a = \frac{1}{6}-o(1)$. The algorithm is not based on memorizing small chunks of data (often used for logarithmic speedups, including the "Four Russians Trick" in LCS), but rather utilizes a new technique, bounding the number of significant symbol matches between the two sequences.

==> short.tex <==
% from STACS preliminary version, unneeded after limit increased to 15 pages
\section{The algorithm -- sketch}
\label{section:algo-sketch}
In this section we introduce our algorithm for computing LCIS, which is based on the bounds for significant pairs developed previously. Due to space constraints we only include here the sketch of the algorithm and briefly discuss its complexity, while providing the full version as Appendix \ref{section:algo-full}. We feel that, unlike combinatorial proofs in Section \ref{section:counting}, most of the algorithm analysis is intuitive and straightforward, if a bit technical.

The algorithm uses priority queues which store matching pairs of indices, i.e., pairs $(x,y)$ of integers from the interval $[1..n]$, sorted either by first or second coordinate. Such a queue should also provide basic operations (inserting/finding/removing an element, providing next and previous element) in $\O{\log \log n}$ amortized time complexity. This is achieved by employing van Emde Boas queues \cite{vanEmdeBoas75, MehlhornN90}. The space complexity must be proportional to number of elements stored, and not be $\Om{n}$ -- the version in \cite{MehlhornN90} meets this requirement, though it is randomized. In Appendix \ref{sec:vEB} we propose another variant of van Emde Boas queue, with good enough space complexity as well as fully deterministic.

The algorithm takes, as the input, two integer sequences $A$ and $B$ with $|A| = |B| = n$. Its main idea is to consider all symbols from $A$ and $B$ in increasing order (there are at most $2n$ of them, so we can sort them in $\O{n \log n}$). For every symbol $\sigma$, the algorithm finds and stores all significant $\sigma$-pairs. For that, we employ $n$ van Emde Boas queues $Q_1, Q_2, \ldots, Q_n$, with every $Q_k$ storing the significant pairs $(x,y)$ with $\lcisto{x,y} = k$, sorted by $x$. For convenience, we define $Q = Q_1 \cup \ldots \cup Q_n$. 

Whenever some $Q_k$ contains two pairs $(x,y) \leq (x',y')$, we drop $(x',y')$ from $Q_k$. Informally, we can do it because $(x,y)$ can replace $(x',y')$ in every situation. This leads to the following invariant: 

\begin{claim*}[Algorithm invariant]
For every $k$, all pairs $(x,y) \in Q_k$ are in strict increasing order with respect to $x$ and in strict decreasing order with respect to $y$. 
\end{claim*}

It is straightforward (and explained in full version) to modify the inserting subroutine for all $Q_k$ to keep the invariant at all times. Apart from queues $Q_1, Q_2, \ldots, Q_n$ we will also need, for every symbol $\sigma$, two van Emde Boas queues $X_\sigma$ and $Y_\sigma$ which store positions of all $\sigma$-symbols in $A$ and $B$, respectively: $X_\sigma = \{i : A[i] = \sigma\}$, $Y_\sigma = \{j : B[j] = \sigma\}$. These structures do not change during the algorithm, and their sole purpose is finding $\sigma$-symbols closest to a given position. 

Now we are ready to introduce the main idea of the algorithm. Recall that we assume that the number of significant pairs between $A$ and $B$ is at most $\O{\frac{n^2}{t}}$  with $t = t(n) = \Th{\log^p n}$ for some $p$. We iterate over all the symbols in increasing order, dividing them into two categories:
\begin{itemize}
 \item \emph{frequent} -- appearing more than $\frac{n}{\sqrt{t}}$ times in $B$,
 \item \emph{infrequent} -- with at most $\frac{n}{\sqrt{t}}$ occurrences in $B$.\footnote[3]{The technique of splitting symbols of a string according to their number of occurences is not new -- it has been used, e.g. in \cite{AmirLP00}, though it is more common to have split thresholds closer to $\sqrt{n}$.}
\end{itemize}

 Let us sketch the algorithm behavior for both cases. The frequent symbols are easier: for every such symbol $\sigma$ we iterate through all previously found pairs, and for every $(x,y) \in Q$ we find the next occurrence of $\sigma$ after $A[x]$ (say, $A[x^*]$) and the next occurrence $y^*$ of $\sigma$ in $B$ after $y$. In other words, we find a $\sigma$-pair $(x^*, y^*)$ for which $(x,y)$ is a predecessor. This can be done easily using $X_\sigma$ and $Y_\sigma$ queues. As we ensure that $Q$ contains only significant pairs (and thus cannot be larger than $\O{\frac{n^2}{t}}$) and there are no more than $\sqrt{t}$ frequent symbols, the total complexity is at most $\O{\frac{n^2 \log \log n}{\sqrt{t}}}$, with additional $\log \log n$ factor from queue operations. Informally, as every significant pair has a predecessor that has been found before, we do not miss any $\sigma$-pair this way. The invariant also ensures that no insignificant pair ever appears in $Q$.

Handling infrequent symbols is a bit harder: observe that every such symbol in $A$ can form a matching pair with at most $\frac{n}{\sqrt{t}}$ elements of $B$. Hence, there are at most $\frac{n^2}{\sqrt{t}}$ matching pairs on infrequent symbols, so we can iterate through all of them. The hardest part is to determine, for every infrequent pair $(x,y)$, the value of $\lcisto{x,y}$, to pick the right $Q_k$ for inserting $(x,y)$. For that, we need a separate subroutine \fun{ComputeNextPair}{}, which takes three arguments: positions $x \in A$, $y \in B$, such that $A[x] = B[y] = \sigma$, and an integer $k$. It assumes that all significant pairs for every symbol $\sigma' < \sigma$ are already found, and that $\lcisto{x,y} \geq k$. The goal of the subroutine is to finds the exact value of $\lcisto{x,y}$. Observe that it is equivalent to finding the predecessor of $(x,y)$ -- determining the largest $\ell \geq k-1$ for which there is a pair $(x',y') \prec (x,y)$ with $\lcisto{x',y'} = \ell$. 

We can guess $\ell$, and verify whether there exists a right pair $(x',y') \prec (x,y)$ in $Q_{\ell}$: if there is one, then $\fun{Prev}{Q_{\ell},x} \leq (x,y)$, where $\fun{Prev}{Q_{\ell},x}$ denotes the last element on $Q_{\ell}$ with its first coordinate less than $x$. Also, if some $\ell$ is valid, then all smaller values are valid as well: if $\lcisto{x',y'} = \ell$, then $\lcisto{\prv{x',y'}} = \ell-1$ and $\prv{x',y'} \prec (x,y)$. This allows us to do a binary search for $\ell$, which needs $\log(\ell - k + 2)$ steps.

For fixed $x$, let $y_1, \ldots, y_m$ are all indices such that $B[y_i] = A[x] = \sigma$ for $1 \leq i \leq m$. We make $m$ calls to \fun{ComputeNextPair}{} subroutine, each to determine $\lcisto{x,y_i}$ for some $i$, assuming that it is greater or equal to $\lcisto{x,y_{i-1}}$. Such a call requires a single binary search working in $\log(\lcis{x,y_{i}} - \lcis{x,y_{i-1}} + 2)$ steps. Using Jensen's equality we prove that the total number of steps needed in all calls does not exceed $\O{\frac{n \log \log n} {\sqrt{t}} }$ which, taking into account queue operations and summing over all possible values of $x$, yields the grand total of $\O{\frac{n^2 (\log \log n)^2} {\sqrt{t}}}$ time complexity. 


Summing the complexity for frequent and infrequent symbols, we obtain that Theorem \ref{thm:main-algo} is true: the algorithm indeed works in $\O{\frac{n^2 (\log \log n)^2}{\sqrt{t}}}$ time complexity.


